Better Pay Attention Whilst Fuzzing

Fuzzing is one of the prevailing methods for vulnerability detection. However, even state-of-the-art fuzzing methods become ineffective after some period of time, i.e., the coverage hardly improves as existing methods are ineffective to focus the attention of fuzzing on covering the hard-to-trigger program paths. In other words, they cannot generate inputs that can break the bottleneck due to the fundamental difficulty in capturing the complex relations between the test inputs and program coverage. In particular, existing fuzzers suffer from the following main limitations: 1) lacking an overall analysis of the program to identify the most "rewarding" seeds, and 2) lacking an effective mutation strategy which could continuously select and mutates the more relevant "bytes" of the seeds. In this work, we propose an approach called ATTuzz to address these two issues systematically. First, we propose a lightweight dynamic analysis technique which estimates the "reward" of covering each basic block and selects the most rewarding seeds accordingly. Second, we mutate the selected seeds according to a neural network model which predicts whether a certain "rewarding" block will be covered given certain mutation on certain bytes of a seed. The model is a deep learning model equipped with attention mechanism which is learned and updated periodically whilst fuzzing. Our evaluation shows that ATTuzz significantly outperforms 5 state-of-the-art grey-box fuzzers on 13 popular real-world programs at achieving higher edge coverage and finding new bugs. In particular, ATTuzz achieved 2X edge coverage and 4X bugs detected than AFL over 24-hour runs. Moreover, ATTuzz persistently improves the edge coverage in the long run, i.e., achieving 50% more coverage than AFL in 5 days.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> mot.tex <==
\subsection{A Motivating Example}
\label{sec:mov}

\begin{figure}[t]
{\footnotesize
\begin{verbatim}
            void func(int a, int b, int c, char* buf) {
            1.    int Flag = 0;
            2.    if(a > 100) {
            3.        if(b == -1) {
            4.            if(c < 0) {
            5.    	          Flag = 1;
                             return 0;
                          }
                      }
                  } 
            6.    if(Flag) {
            7.        if(buf[0] == "X") {
            8.            buggy code ...;		
                      }    	
                  }
            9.    return 1;
              }
\end{verbatim}}
\caption{A motivating example}
\label{mot}
\end{figure}
% \todo{It would make a much better impression if the example can be some real bug - even better some CVE.}In this section, we use a simple program (shown in Figure~\ref{mot}) to illustrate the motivation of our work. 
% Figure~\ref{motivating} shows a concrete code snippet of our motivating example.The code segment itself is very simple. 
We start with a motivating example shown in Figure~\ref{mot}. First, the program checks a nested condition determined by three variables $a$, $b$, and $c$. The $Flag$ is set to 1 if the nested condition is satisfied. Then, the program determines if the corresponding bytes in the buffer are equal to $X$. If yes, a bug is triggered.
% When all the conditions are met, we can reach the real functional module, where bugs often hide.

% What is the problem if we use AFL to fuzz such a program fragment? 
Such a simple program brings several challenges to coverage-guided fuzzers like AFL. First, \emph{the nested conditions and checksum are not easy to be satisfied by random mutations (Challenge 1),} i.e., the probability to generate a seed covering new control locations is extremely low. Second, even if we finally meet the conditions and obtain the corresponding seed, \emph{the effectiveness of the seed will be easily destroyed by the random mutation mechanisms (Challenge 2).} 
For example, after a period of fuzzing, AFL finally met the conditions of line 2, 3 and 4 in Figure~\ref{mot}, and obtained a seed file that can set $Flag$ to 1. In order to further improve coverage, AFL mutates this seed to generate more inputs. Unfortunately, such random mutations are hardly useful as they very likely set flag to false. For instance, AFL fails to cover line 8 after 12 hours and 13 million runs even a seed which could set $Flag$ to 1 is given.  
% \sj{Provide some statistics here to support the argument - like AFL failed to cover the branch in 2 hours ... }
% For AFL, even after giving a seed file that can set Flag to 1, after 12h fuzzing and 13 million runs, it cannot reach 8 lines. First, AFL still uses the default strategy to select seed files from the massive seed file pool. As a result, only 8\% of the seed files selected by AFL can set the flag to 1 after the seed files reaching line 7 are successfully generated. What's more, the random mutation strategy results in that even if the correct seed file is selected, only 1.3\% of the newly generated input can still reach line 7

% For example, a simple $bitflip$ can change the value from a positive number to a negative number, causing the condition in the line 4 of the Figure~\ref{motivating} to not be met. Even if we successfully meet the condition of the 7 row of the function, we still cannot reach the target basic block because we have destroyed the condition of the flag. In response to this problem, we proposed our strategy to make the mutation efficient through guidance.

To tackle the above challenges, different works have been proposed which can be roughly divided into two categories.
% To solve this problem, the methods proposed by the existing work can be roughly divided into two categories. 
The first category used program analysis techniques such as dynamic taint analysis~\cite{rawat2017vuzzer,chen2018angora}, concolic execution~\cite{stephens2016driller,yun2018qsym,cadar2008klee,king1976symbolic} and static analysis~\cite{li2017steelix, rawat2017vuzzer} to identify the most relevant bytes to mutate (a.k.a. solving the magic byte problem) directly. While program analysis based approaches can accurately obtain the value of the magic byte (with a powerful solver at hand), the subsequent mutation may still destroy such ``magic''. The other category introduced machine learning to filter less meaningful inputs (potentially with no coverage gain)~\cite{zong2020fuzzguard} or use it to generate more valuable inputs~\cite{rajpal2017not, she2019neuzz}. However, existing machine learning based approaches have limited effectiveness in selecting control locations that can maximize the coverage reward. For instance, Neuzz's gradient guided mutation strategy can only keep 10\% of newly generated inputs reaching line 7 with seeds setting $Flag$ to 1. Besides, the adopted machine learning models (e.g., LSTM~\cite{rajpal2017not} and NN~\cite{she2019neuzz}) are often considered lacking of interpretability.
% 
% \sj{similarly, provide some statistics here to support the argument - like neFuzz failed to cover ...}

% Similarly Neuzz uses a seed selection strategy similar to that of AFL, so although it has gradient-guided mutation, only about 10\% of newly generated inputs can set flag to 1 after reach reaching line 7.
 
% still cause the input to fail to execute to the target code segment.   
% [RNNfuzzer][Neuzz].
% It is true that the method of program analysis can accurately obtain the specific value of the magic byte, but as mentioned earlier, even if the magic byte is satisfied, the mutation strategy may still cause the input to fail to execute to the target code segment.
% [RNNfuzzer] does not give a method for selecting the nodes that need training, while [Neuzz] learns the overall CFG of the program. The method they proposed reduces the possibility of destroying the previous conditions to a certain extent, but makes the input control flow lacks directivity.

% Our method can break through the key basic blocks that have not yet been covered without destroying the prerequisites, so as to improve the overall coverage of the program more efficiently.

In this work, we aim to address both challenges systematically by deepening our understanding from two sides, i.e., the program and the fuzzing process, and their interactions. First, we use a carrier fuzzer (e.g., AFL) to generate a number of tests and run the target program with them. Note that the program is instrumented to collect the execution trace of each input, which contains more fine-grained information than coverage. After a while, \tool determines that covering some of the blocks that are yet to be covered will be more rewarding than others by calculating a \emph{coverage reward} for each uncovered control locations based on the abstraction of the program estimated from the fuzzing data. In the running example, line 7 will have the highest reward. 
%as it will trigger the buggy code. 
\tool then selects the target control locations for machine learning by prioritizing those with high rewards. In the machine learning phase, \tool adopts state-of-the-art deep learning models with attention mechanism, which allows us not only to predict whether a specific combination of seed and mutator can reach the target location, but also to obtain the ``explanation'' (in form of heat maps) which informs us the importance of different bytes (under a mutator) on the program coverage (e.g., can reach line 7 or not). With the explanation, \tool then guides the fuzzer to mutate the corresponding position of the input with different probabilities. In the example, if the seed input can already set $Flag$ to 1, we will avoid performing $bitflip$ on $b$, and allow $arth$ to operate on $c$. In this way, the effectiveness of the seeds will be preserved and many more inputs satisfying the nested conditions in line 2, 3 and 4 will be generated, thereby increasing the probability of triggering the bug in line 8.

% breaking the bottleneck of row 9 instead of generating a large number of invalid inputs based on seeds. 
% Finally, in the updating phrase, XXX performs the above steps for newly encountered uncovered blocks to maximize the entire program's coverage. Below we provide the details of these modules.  

% In the model training phase, in addition to simple classification, XXX adds an attention mechanism, which allows us not only to predict whether the combination of seed and mutation can trigger the target block but also to obtain \textbf{heat maps} which tells us that performing different mutations to the variable $a$, $b$, $c$, and $buf$ will affect whether the program can execute to line 7. 

% In the \textbf{mutation strategy updating phrase}, according to the heat maps of different mutators, XXX guides the fuzzer to mutate the corresponding position of the input with different probabilities. For example, for the fragment in figure~\ref{motivating}, if the seed file can already set the flag to one, we will avoid performing $bitflip$ operations on the variable $b$, and allow $arth-$ to operate on the variable $c$. In this way, we can generate rich input while ensuring that the conditions of rows 2, 3, and 4 in figure~\ref{motivating} are met, thereby breaking the bottleneck of row 9 instead of generating a large number of invalid inputs based on seeds. 
% Finally, in the updating phrase, XXX performs the above steps for newly encountered uncovered blocks to maximize the entire program's coverage. Below we provide the details of these modules.


